Channel Estimation Techniques for Diffusion-Based Molecular Communications

In molecular communication (MC) systems, the expected number of molecules observed at the receiver over time after the instantaneous release of molecules by the transmitter is referred to as the channel impulse response (CIR). Knowledge of the CIR is needed for the design of detection and equalization schemes. In this paper, we present a training-based CIR estimation framework for MC systems which aims at estimating the CIR based on the observed number of molecules at the receiver due to emission of a sequence of known numbers of molecules by the transmitter. In particular, we derive maximum likelihood (ML) and least sum of square errors (LSSE) estimators. We also study the Cramer Rao (CR) lower bound and training sequence design for the considered system. Simulation results confirm the analysis and compare the performance of the proposed estimation techniques with the CR lower bound.

==> Fig/BayesianCIR/BayesianCIR.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA LSSE Estimation\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA MMSE Estimation\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA Bayesian CR Bound\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextB $\sigma^2 = 0.1$}%
\psfrag{020}[cl][cl]{\matlabtextB $\sigma^2 = 0.01$}%
\psfrag{021}[bc][bc]{\matlabtextB Normalized Estimaion Error (dB)}%
\psfrag{022}[tc][tc]{\matlabtextB Sequence Length $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $20$}%
\psfrag{002}[ct][ct]{\matlabtextC $40$}%
\psfrag{003}[ct][ct]{\matlabtextC $60$}%
\psfrag{004}[ct][ct]{\matlabtextC $80$}%
\psfrag{005}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $-28$}%
\psfrag{007}[rc][rc]{\matlabtextC $-26$}%
\psfrag{008}[rc][rc]{\matlabtextC $-24$}%
\psfrag{009}[rc][rc]{\matlabtextC $-22$}%
\psfrag{010}[rc][rc]{\matlabtextC $-20$}%
\psfrag{011}[rc][rc]{\matlabtextC $-18$}%
\psfrag{012}[rc][rc]{\matlabtextC $-16$}%
\psfrag{013}[rc][rc]{\matlabtextC $-14$}%
\psfrag{014}[rc][rc]{\matlabtextC $-12$}%
\psfrag{015}[rc][rc]{\matlabtextC $-10$}%
%
%% </ytick>

==> Fig/DeterSeq/DeterSeq.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA CR Lower Bound\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA ML Estimation\hspace{0.5em}}%
\psfrag{019}[cl][cl]{\matlabtextA LSSE Estimation\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextB $L=5$}%
\psfrag{021}[cl][cl]{\matlabtextB $L=3$}%
\psfrag{022}[cl][cl]{\matlabtextB $L=1$}%
\psfrag{023}[bc][bc]{\matlabtextB Normalized Estimaion Error Variance, $ \overline{\mathrm{Var}}_{\mathbf{e}}$, in dB}%
\psfrag{024}[tc][tc]{\matlabtextB Sequence Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10$}%
\psfrag{001}[ct][ct]{\matlabtextC $20$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $40$}%
\psfrag{004}[ct][ct]{\matlabtextC $50$}%
\psfrag{005}[ct][ct]{\matlabtextC $60$}%
\psfrag{006}[ct][ct]{\matlabtextC $70$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $90$}%
\psfrag{009}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $-30$}%
\psfrag{011}[rc][rc]{\matlabtextC $-25$}%
\psfrag{012}[rc][rc]{\matlabtextC $-20$}%
\psfrag{013}[rc][rc]{\matlabtextC $-15$}%
\psfrag{014}[rc][rc]{\matlabtextC $-10$}%
\psfrag{015}[rc][rc]{\matlabtextC $-5$}%
\psfrag{016}[rc][rc]{\matlabtextC $0$}%
%
%% </ytick>

==> Fig/Error/Error.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{060}[tc][tc]{\matlabtextA Index of Realization of $\mathbf{r}$ for CIR Estimation}%
\psfrag{061}[bc][bc]{\matlabtextA LSSE Estimation, $K=80$}%
\psfrag{062}[bc][bc]{\matlabtextA Estimated CIR}%
\psfrag{063}[bc][bc]{\matlabtextA ML Estimation, $K=80$}%
\psfrag{064}[bc][bc]{\matlabtextA LSSE Estimation, $K=20$}%
\psfrag{065}[bc][bc]{\matlabtextA ML Estimation, $K=20$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $100$}%
\psfrag{002}[ct][ct]{\matlabtextB $200$}%
\psfrag{003}[ct][ct]{\matlabtextB $300$}%
\psfrag{004}[ct][ct]{\matlabtextB $400$}%
\psfrag{005}[ct][ct]{\matlabtextB $500$}%
\psfrag{006}[ct][ct]{\matlabtextB $600$}%
\psfrag{007}[ct][ct]{\matlabtextB $700$}%
\psfrag{008}[ct][ct]{\matlabtextB $800$}%
\psfrag{009}[ct][ct]{\matlabtextB $900$}%
\psfrag{010}[ct][ct]{\matlabtextB $1000$}%
\psfrag{015}[ct][ct]{\matlabtextB $0$}%
\psfrag{016}[ct][ct]{\matlabtextB $100$}%
\psfrag{017}[ct][ct]{\matlabtextB $200$}%
\psfrag{018}[ct][ct]{\matlabtextB $300$}%
\psfrag{019}[ct][ct]{\matlabtextB $400$}%
\psfrag{020}[ct][ct]{\matlabtextB $500$}%
\psfrag{021}[ct][ct]{\matlabtextB $600$}%
\psfrag{022}[ct][ct]{\matlabtextB $700$}%
\psfrag{023}[ct][ct]{\matlabtextB $800$}%
\psfrag{024}[ct][ct]{\matlabtextB $900$}%
\psfrag{025}[ct][ct]{\matlabtextB $1000$}%
\psfrag{030}[ct][ct]{\matlabtextB $0$}%
\psfrag{031}[ct][ct]{\matlabtextB $100$}%
\psfrag{032}[ct][ct]{\matlabtextB $200$}%
\psfrag{033}[ct][ct]{\matlabtextB $300$}%
\psfrag{034}[ct][ct]{\matlabtextB $400$}%
\psfrag{035}[ct][ct]{\matlabtextB $500$}%
\psfrag{036}[ct][ct]{\matlabtextB $600$}%
\psfrag{037}[ct][ct]{\matlabtextB $700$}%
\psfrag{038}[ct][ct]{\matlabtextB $800$}%
\psfrag{039}[ct][ct]{\matlabtextB $900$}%
\psfrag{040}[ct][ct]{\matlabtextB $1000$}%
\psfrag{045}[ct][ct]{\matlabtextB $0$}%
\psfrag{046}[ct][ct]{\matlabtextB $100$}%
\psfrag{047}[ct][ct]{\matlabtextB $200$}%
\psfrag{048}[ct][ct]{\matlabtextB $300$}%
\psfrag{049}[ct][ct]{\matlabtextB $400$}%
\psfrag{050}[ct][ct]{\matlabtextB $500$}%
\psfrag{051}[ct][ct]{\matlabtextB $600$}%
\psfrag{052}[ct][ct]{\matlabtextB $700$}%
\psfrag{053}[ct][ct]{\matlabtextB $800$}%
\psfrag{054}[ct][ct]{\matlabtextB $900$}%
\psfrag{055}[ct][ct]{\matlabtextB $1000$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextB $0$}%
\psfrag{012}[rc][rc]{\matlabtextB $10$}%
\psfrag{013}[rc][rc]{\matlabtextB $20$}%
\psfrag{014}[rc][rc]{\matlabtextB $30$}%
\psfrag{026}[rc][rc]{\matlabtextB $0$}%
\psfrag{027}[rc][rc]{\matlabtextB $10$}%
\psfrag{028}[rc][rc]{\matlabtextB $20$}%
\psfrag{029}[rc][rc]{\matlabtextB $30$}%
\psfrag{041}[rc][rc]{\matlabtextB $0$}%
\psfrag{042}[rc][rc]{\matlabtextB $10$}%
\psfrag{043}[rc][rc]{\matlabtextB $20$}%
\psfrag{044}[rc][rc]{\matlabtextB $30$}%
\psfrag{056}[rc][rc]{\matlabtextB $0$}%
\psfrag{057}[rc][rc]{\matlabtextB $10$}%
\psfrag{058}[rc][rc]{\matlabtextB $20$}%
\psfrag{059}[rc][rc]{\matlabtextB $30$}%
%
%% </ytick>

==> Fig/ISI/ISI.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[bc][bc]{\matlabtextA b)}%
\psfrag{001}[bc][bc]{\matlabtextA Expected number of observed molecules}%
\psfrag{002}[tc][tc]{\matlabtextA Time (ms)}%
\psfrag{003}[tl][tl]{\matlabtextA \begin{tabular}{@{}l@{}}Desired\\Component\end{tabular}}%
\psfrag{004}[tl][tl]{\matlabtextA \begin{tabular}{@{}l@{}}ISI\\Components\end{tabular}}%
%
%% </text>

==> Fig/MeanDet/MeanDet.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA ML Estimation\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA LSSE Estimation\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextB $L=5$}%
\psfrag{020}[cl][cl]{\matlabtextB $L=3$}%
\psfrag{021}[cl][cl]{\matlabtextB $L=1$}%
\psfrag{022}[bc][bc]{\matlabtextB Normalized Estimaion Error Mean, $ \overline{\mathrm{Mean}}_{\mathbf{e}}$, in dB}%
\psfrag{023}[tc][tc]{\matlabtextB Sequence Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10$}%
\psfrag{001}[ct][ct]{\matlabtextC $20$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $40$}%
\psfrag{004}[ct][ct]{\matlabtextC $50$}%
\psfrag{005}[ct][ct]{\matlabtextC $60$}%
\psfrag{006}[ct][ct]{\matlabtextC $70$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $90$}%
\psfrag{009}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $-70$}%
\psfrag{011}[rc][rc]{\matlabtextC $-60$}%
\psfrag{012}[rc][rc]{\matlabtextC $-50$}%
\psfrag{013}[rc][rc]{\matlabtextC $-40$}%
\psfrag{014}[rc][rc]{\matlabtextC $-30$}%
\psfrag{015}[rc][rc]{\matlabtextC $-20$}%
\psfrag{016}[rc][rc]{\matlabtextC $-10$}%
%
%% </ytick>

==> Fig/SeqDes/SeqDes.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{022}[cl][cl]{\matlabtextA ISI-Free Sequence, Simulation Result\hspace{0.5em}}%
\psfrag{023}[cl][cl]{\matlabtextA Optimal Sequence, Simulation Result\hspace{0.5em}}%
\psfrag{024}[cl][cl]{\matlabtextA ISI-Free Sequence, Analytical Upper Bound in (17)\hspace{0.5em}}%
\psfrag{025}[cl][cl]{\matlabtextA Optimal Sequence, Analytical Upper Bound in (17)\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{026}[cl][cl]{\matlabtextB $L=5$}%
\psfrag{027}[cl][cl]{\matlabtextB $L=3$}%
\psfrag{028}[cl][cl]{\matlabtextB $L=2$}%
\psfrag{029}[cl][cl]{\matlabtextB $L=1$}%
\psfrag{030}[bc][bc]{\matlabtextB Normalized Estimaion Error Variance, $ \overline{\mathrm{Var}}_{\mathbf{e}}$, in dB}%
\psfrag{031}[tc][tc]{\matlabtextB Sequence Length $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $2$}%
\psfrag{001}[ct][ct]{\matlabtextC $4$}%
\psfrag{002}[ct][ct]{\matlabtextC $6$}%
\psfrag{003}[ct][ct]{\matlabtextC $8$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
\psfrag{005}[ct][ct]{\matlabtextC $12$}%
\psfrag{006}[ct][ct]{\matlabtextC $14$}%
\psfrag{007}[ct][ct]{\matlabtextC $16$}%
\psfrag{008}[ct][ct]{\matlabtextC $18$}%
\psfrag{009}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $-22$}%
\psfrag{011}[rc][rc]{\matlabtextC $-20$}%
\psfrag{012}[rc][rc]{\matlabtextC $-18$}%
\psfrag{013}[rc][rc]{\matlabtextC $-16$}%
\psfrag{014}[rc][rc]{\matlabtextC $-14$}%
\psfrag{015}[rc][rc]{\matlabtextC $-12$}%
\psfrag{016}[rc][rc]{\matlabtextC $-10$}%
\psfrag{017}[rc][rc]{\matlabtextC $-8$}%
\psfrag{018}[rc][rc]{\matlabtextC $-6$}%
\psfrag{019}[rc][rc]{\matlabtextC $-4$}%
\psfrag{020}[rc][rc]{\matlabtextC $-2$}%
\psfrag{021}[rc][rc]{\matlabtextC $0$}%
%
%% </ytick>

==> Fig/SeqISIFree/SeqISIFree.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA ISIF\hspace{0.5em}}%
\psfrag{019}[cl][cl]{\matlabtextA LSSE\hspace{0.5em}}%
\psfrag{020}[cl][cl]{\matlabtextA MMSE\hspace{0.5em}}%
\psfrag{021}[cl][cl]{\matlabtextA ML\hspace{0.5em}}%
\psfrag{022}[cl][cl]{\matlabtextA CRB\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[bc][bc]{\matlabtextB Normalized Estimaion Error (dB)}%
\psfrag{024}[tc][tc]{\matlabtextB Sequence Length $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $20$}%
\psfrag{001}[ct][ct]{\matlabtextC $30$}%
\psfrag{002}[ct][ct]{\matlabtextC $40$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
\psfrag{005}[ct][ct]{\matlabtextC $70$}%
\psfrag{006}[ct][ct]{\matlabtextC $80$}%
\psfrag{007}[ct][ct]{\matlabtextC $90$}%
\psfrag{008}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $-32$}%
\psfrag{010}[rc][rc]{\matlabtextC $-30$}%
\psfrag{011}[rc][rc]{\matlabtextC $-28$}%
\psfrag{012}[rc][rc]{\matlabtextC $-26$}%
\psfrag{013}[rc][rc]{\matlabtextC $-24$}%
\psfrag{014}[rc][rc]{\matlabtextC $-22$}%
\psfrag{015}[rc][rc]{\matlabtextC $-20$}%
\psfrag{016}[rc][rc]{\matlabtextC $-18$}%
\psfrag{017}[rc][rc]{\matlabtextC $-16$}%
%
%% </ytick>
